Characterizing Transaction-Reverting Statements in Ethereum Smart Contracts

Smart contracts are programs running on blockchain to execute transactions. When input constraints or security properties are violated at runtime, the transaction being executed by a smart contract needs to be reverted to avoid undesirable consequences. On Ethereum, the most popular blockchain that supports smart contracts, developers can choose among three transaction-reverting statements (i.e., require, if...revert, and if...throw) to handle anomalous transactions. While these transaction-reverting statements are vital for preventing smart contracts from exhibiting abnormal behaviors or suffering malicious attacks, there is limited understanding of how they are used in practice. In this work, we perform the first empirical study to characterize transaction-reverting statements in Ethereum smart contracts. We measured the prevalence of these statements in 3,866 verified smart contracts from popular dapps and built a taxonomy of their purposes via manually analyzing 557 transaction-reverting statements. We also compared template contracts and their corresponding custom contracts to understand how developers customize the use of transaction-reverting statements. Finally, we analyzed the security impact of transaction-reverting statements by removing them from smart contracts and comparing the mutated contracts against the original ones. Our study led to important findings, which can shed light on further research in the broad area of smart contract quality assurance and provide practical guidance to smart contract developers on the appropriate use of transaction-reverting statements.

==> tables/RQ1/var_type_classification.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
    \caption{Variable type involved in require statement}
    \label{var type}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|p{3cm}|p{4cm}|p{9cm}|}
    \hline
    Category                        & Sub-Category             & Description                                                                              \\ \hline

    \multirow{2}{*}{State Variable} & Common State Variable    & Variables whose values are permanently stored in a contract storage.                     \\ \cline{2-3} 
                                    & Address-related Variable & Variables whose values are related to contract addresses, including address and balance. \\ \hline
    \multirow{4}{*}{Local Variable} & Identifier               & \multirow{4}{*}{Variables whose values are present till function is executing.}          \\ \cline{2-2}
                                    & ElementaryTypeName       &                                                                                          \\ \cline{2-2}
                                    & MemberAccess             &                                                                                          \\ \cline{2-2}
                                    & ...                      &                                                                                          \\ \hline
    Block and Transaction Variable &  & Special variables exists in the global namespace used to get information about the blockchain. \\ \hline
    \end{tabular}%
    }
    \end{table*}

==> tables/RQ3/100_sample_frequent_patterns_result.tex <==

\begin{table}[]

\caption{The distribution of Frequent-changed patterns for 100 random samples}
\label{100samples}

\centering

\begin{tabular}{|l|l|l|}
\hline
\multicolumn{2}{|l|}{Frequent-changed Pattern}                    & Count \\ \hline
\multirow{3}{*}{Add}    & Add transaction-reverting statements    & 52    \\ \cline{2-3} 
                        & Add clauses                             & 1     \\ \cline{2-3} 
                        & Add variables                           & 2     \\ \hline
\multirow{3}{*}{Delete} & Delete transaction-reverting statements & 17    \\ \cline{2-3} 
                        & Delete clauses                          & 3     \\ \cline{2-3} 
                        & Delete variables                        & 2     \\ \hline
\multirow{2}{*}{Modify} & Modify statement types                  & 0     \\ \cline{2-3} 
                        & Modify clauses                          & 7     \\ \hline
Other                   & Format modification                     & 16    \\ \hline
\multicolumn{2}{|l|}{Total}                                       & 112   \\ \hline
\end{tabular}
\end{table}

==> tables/RQ3/code_clone_result.tex <==
\begin{table}[]

\caption{Code Clone Result}
\label{Code Clone Result}

\centering

\begin{tabular}{lcc}
\hline
                    & Similar Contracts & Similar Libraries \\ \hline
dapp contracts     & 175               & 63                  \\
Ethereum contracts & 19,328            & 2,239             \\
Total              & 19,503            & 2,302                  \\ \hline
\end{tabular}
\end{table}

==> tables/RQ4/SWC_result.tex <==
\begin{table}[]

\caption{Known weaknesses Detection Results}
\label{swc_result}

\centering

\begin{tabular}{ccccc}
\hline
\multirow{2}{*}{SWC} & \multicolumn{2}{c}{Template Contract} & \multicolumn{2}{c}{Dapp Contract} \\ \cline{2-5} 
                        & Count            & Percentage          & Count            & Percentage        \\ \hline
SWC-101              & 9/270            & 3.33\%              & 503/3866         & 13.01\%           \\ 
SWC-104              & 2/270            & 0.07\%              & 51/3866          & 1.32\%            \\ 
SWC-105              & 0/270            & 0.00\%              & 17/3866          & 0.44\%            \\ 
SWC-106              & 0/270            & 0.00\%              & 8/3866           & 0.21\%            \\ 
SWC-110              & 0/270            & 0.00\%              & 7/3866           & 0.18\%            \\ 
SWC-123              & 8/270            & 2.96\%              & 729/3866         & 18.86\%           \\ 
SWC-132              & 0/270            & 0.00\%              & 3/3866           & 0.07\%            \\ 
SWC-135              & 15/270           & 5.55\%              & 943/3866         & 24.39\%           \\ \hline
\end{tabular}
\end{table}

==> tables/RQ4/dasp_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]

% \small
\normalsize
% \large

\caption{Number of Vulnerabilities Reported by Nine Analysis Tools on Original and Mutated Contracts}
\label{DASP running results}

\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|r|r|r|r|r|r|r|r|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{Tools}} & \multicolumn{8}{c|}{\# Vulnerabilities in Different Types} \\ \cline{3-10} 
\multicolumn{2}{|l|}{}      & Access Control & Arithmetic & Denial Service & Reentracy & Uncheck Low Calls & Front Running & Time Manipulation & Unknown Unknowns \\ \hline
\multirow{2}{*}{Slither}     & Original & 470   & /     & 744  & 3049 & 845   & /     & 400 & 1562   \\ \cline{2-10} 
                            & Mutated  & 462   & /     & 741  & 3026 & 833   & /     & 395 & 1547   \\ \hline
\multirow{2}{*}{Securify}    & Original & 12988 & /     & /    & 1630 & 14938 & 18663 & /   & /      \\ \cline{2-10} 
                            & Mutated  & 13812 & /     & /    & 1574 & 14624 & 20244 & /   & /      \\ \hline
\multirow{2}{*}{Manticore}   & Original & 26    & 41    & /    & 10   & 0     & /     & 60  & 442    \\ \cline{2-10} 
                            & Mutated  & 34    & 101   & /    & 0    & 2     & /     & 62  & 696    \\ \hline
\multirow{2}{*}{Maian}       & Original & 7714  & /     & /    & /    & /     & /     & /   & 3857   \\ \cline{2-10} 
                            & Mutated  & 7714  & /     & /    & /    & /     & /     & /   & 3857   \\ \hline
\multirow{2}{*}{Honeybadger} & Original & /     & /     & /    & /    & /     & /     & /   & 9      \\ \cline{2-10} 
                            & Mutated  & /     & /     & /    & /    & /     & /     & /   & 7      \\ \hline
\multirow{2}{*}{Oyente}      & Original & 0     & 17005 & 135  & 26   & /     & /     & 118 & /      \\ \cline{2-10} 
                            & Mutated  & 0     & 16299 & 136  & 24   & /     & /     & 127 & /      \\ \hline
\multirow{2}{*}{Osiris}      & Original & /     & 3453  & 64   & 41   & /     & /     & 182 & /      \\ \cline{2-10} 
                            & Mutated  & /     & 3379  & 69   & 30   & /     & /     & 179 & /      \\ \hline
\multirow{2}{*}{Mythril}     & Original & 98    & 2443  & /    & 974  & 59    & 297   & /   & 1070   \\ \cline{2-10} 
                            & Mutated  & 94    & 2428  & /    & 956  & 55    & 290   & /   & 1059   \\ \hline
\multirow{2}{*}{Smartcheck}  & Original & 129   & 4009  & 7796 & 183  & 2596  & /     & /   & 181822 \\ \cline{2-10} 
                            & Mutated  & 128   & 4005  & 7794 & 182  & 2573  & /     & /   & 177752 \\ \hline
\end{tabular}%
}
\begin{tablenotes}
\item[1] ``/" represents that this kind of security vulnerability can not be detected by the tool. ``0" represents the number of the vulnerability is zero.
\end{tablenotes}
\end{table*}

==> tables/RQ4/know_weakness.tex <==
\begin{table*}[]

\caption{Known weaknesses related to transaction-reverted statement}
\label{Known weaknesses related to require statement}

\resizebox{\textwidth}{!}{%
\begin{tabular}{|p{4cm}|p{6cm}|p{5cm}|}
\hline
SWC related to transaction-reverting statements & Description                                                                                                      & Purpose tags                            \\ \hline
SWC-101: Integer Overflow and Underflow         & An arithmetic operation reaches the maximum or minimum size of a type.                                           & Legality Check-Overflow/Underflow Check \\ \hline
SWC-104: Unchecked Call Return Value            & The return value of a message call is not checked.                                                               & Legality Check-Logic Check             \\ \hline
SWC-105: Unprotected Ether Withdrawal           & Missing transaction-reverting statements to control the access of ether withdrawal functions.                    & Authority Check-Address Check                  \\ \hline
SWC-106: Unprotected \texttt{SELFDESTRUCT} Instruction   & Missing transaction-reverting statements to control the access of selfdestruct() functions.                        & Authority Check-Address Check                  \\ \hline
% SWC-107: Reentrancy                             & Malicious contract calls back into the calling contract before the first invocation of the function is finished. & Legality Return Value Check             \\ \hline
SWC-110: Assert Violation                       & Trigger the \texttt{assert} statements by wrongly using \texttt{assert} to check variables or triggering bugs.                 & Wrong use of \texttt{assert} and \texttt{require}         \\ \hline
SWC-123: Requirement Violation                  & Invalid input for a transaction-reverting statement.                                                             & Legality Check-Logic Check                          \\ \hline
SWC-132: Unexpected Ether balance               & Contracts strictly assume a specific Ether balance and induce erroneous behavior.                                & Legality Check-Logic Check                          \\ \hline
SWC-135: Code With No Effects                   & Code that does not produce the intended effects and not return a warning.                                        & Legality Check-Logic Check             \\ 
\hline
\end{tabular}
}
\end{table*}

==> tables/RQ4/oyente_result_change.tex <==
\begin{table}[]

\centering
\begin{threeparttable}[ht]
    \caption{The number of Vulnerability Changes for Oyente} 
    \label{oyente_result}

    \begin{tabular}{lccc}
    \hline
    & \#Same & \#Increase & \#Decrease \\ \hline
    EVM Code Coverage                    & 3855     & 0        & 0        \\ 
    Integer Underflow                    & 3714     & 59       & 82       \\ 
    Integer Overflow                     & 3487     & 182      & 186      \\ 
    Parity Multisig Bug 2                & 3855     & 0        & 0        \\ 
    Callstack Depth Attack Vulnerability & 3846     & 6        & 3        \\ 
    Transaction-Ordering Dependency      & 3822     & 14       & 19       \\ 
    Timestamp Dependency                 & 3840     & 7        & 8        \\ 
    Re-Entrancy Vulnerability            & 3854     & 0        & 1        \\ \hline
    \end{tabular}

    Column ``Same'', ``Increase'' and ``Decrease'' presents that the number of contracts in which the number of reported vulnerabilities remains the same, increases and decreases, respectively, after removing transaction-reverting statements.

\end{threeparttable}
\end{table}
